GSDiff: Synthesizing Vector Floorplans via Geometry-enhanced Structural Graph Generation

Automating architectural floorplan design is vital for housing and interior design, offering a faster, cost-effective alternative to manual sketches by architects. However, existing methods, including rule-based and learning-based approaches, face challenges in design complexity and constrained generation with extensive post-processing, and tend to obvious geometric inconsistencies such as misalignment, overlap, and gaps. In this work, we propose a novel generative framework for vector floorplan design via structural graph generation, called GSDiff, focusing on wall junction generation and wall segment prediction to capture both geometric and semantic aspects of structural graphs. To improve the geometric rationality of generated structural graphs, we propose two innovative geometry enhancement methods. In wall junction generation, we propose a novel alignment loss function to improve geometric consistency. In wall segment prediction, we propose a random self-supervision method to enhance the model's perception of the overall geometric structure, thereby promoting the generation of reasonable geometric structures. Employing the diffusion model and the Transformer model, as well as the geometry enhancement strategies, our framework can generate wall junctions, wall segments and room polygons with structural and semantic information, resulting in structural graphs that accurately represent floorplans. Extensive experiments show that the proposed method surpasses existing techniques, enabling free generation and constrained generation, marking a shift towards structure generation in architectural design. Code and data are available at https://github.com/SizheHu/GSDiff.

==> src/3-preliminary.tex <==
\section{Preliminary} 

\paragraph{Diffusion model.}

Diffusion models are a class of generative models training a neural network to adeptly reverse the noise addition process, thereby enabling the generation of data that mimics the original distribution from simple noise. A standard diffusion model generally contains the forward and backward processes.
%
The forward process incrementally adds noise to an original data sample $x_0$ over $T$ steps, resulting in a sample resembling Gaussian noise. For a given step $t$, this process generates a noisier version $x_t$ using:
\begin{equation}
\label{ddpm-forward}
x_t = \sqrt{\gamma_t}x_0 + \sqrt{1-\gamma_t}\epsilon
\end{equation}
where $\gamma_t$ is a noise schedule decreasing from 1 to 0, and $\epsilon$ represents random Gaussian noise.
%
The reverse process starts with the Gaussian noise and progressively denoises it to reconstruct the original data sample $x_0$. The model, through a neural network, estimates less noisy versions of the data step by step, effectively inverting the noise addition from the forward process.
\begin{equation}
p_{\theta}(x_{t-1}|x_t) = \mathcal{N}(x_{t-1}; \frac{\hat{x}_0}{\sqrt{\gamma_t}}, \frac{1-\gamma_t}{\gamma_t}I). \label{ddpm-reverse}
\end{equation}
where $\hat{x}_0 = {x_t - \sqrt{(1-\gamma_t)}\epsilon_{\theta}}$ according to equation \ref{ddpm-forward}.

\paragraph{Representation.}

\begin{figure*}
	\includegraphics[width=0.92\textwidth]{fig/teaser}
	\centering
	\caption{We represent floorplans as structural graphs, generating the node set of the structural graph using diffusion model. Each node's attributes include its positional coordinates and semantic labels of surrounding rooms, ensuring the generated floorplans has accurate room structures and semantics. We subsequently predict the existence of edges between each pair of nodes, and finally extract rooms represented by polygons with semantic labels, resulting in vector floorplans.}
	\label{fig:teaser}
\end{figure*}

We represent the vector floorplan as a structural graph~\cite{sun2022wallplan}: wall junctions are abstracted as nodes, and wall segments as edges. We represent the structural graph as \(G = (V, E)\), where \(V = \{v_1, \ldots, v_n\}\) is the node set, and \(E = \{(v_i, v_j) | v_i, v_j \in V\}\) is the edge set.
%
As shown in the right inset, a node can be denoted as \(v_i = (c_i, r_i, b_i)\), where \(c_i = (x_i, y_i) \in \mathbb{R}^2\) is the positional coordinate. \(r_i \in [0, 1]^n\) denotes the semantics of all rooms that surround \(v_i\), where 0 for absence and 1 for presence of the specific room category, and \(n\) is the number of room categories, which is 7 (\textit{Living room}, \textit{Bedroom}, \textit{Kitchen}, \textit{Bathroom}, \textit{Balcony}, \textit{Storage}, \textit{External area}) in our experiments. 
%
Let \(F = \{R_1, R_2, \ldots, R_m\}\) represent all polygonal loops of rooms, each loop \(R_i = \{v_{i,1}, v_{i,2}, \ldots, v_{i,N_i} | v_{i,j} \in V\}\) is defined by a sequence of graph nodes. The room category of \(R_i\) is the shared room category of all graph nodes forming that room.
%
We have improved the representation of \cite{sun2022wallplan}: (i) For the node set, we set a fixed maximum node number \(N\) by considering background nodes (i.e., without coordinates and semantics) to solve the issue of the uncertain number of nodes in each graph. (ii) We filter out background nodes by adding a background attribute for each node, denoted as \(b_i \in \{0, 1\}\), where 0 denotes the wall junction node and 1 denotes the background node.
%
Vector floorplans have a multi-level structure. Spatially, 0D wall junctions form 1D wall segments, which close into 2D rooms. Semantically, each wall junction that forms a room has the same room semantics. Therefore, generating all 0D wall junctions basically determines the whole floorplan structures. The advantage of this approach is that it preserves all the information of the floorplan by means of 0D wall junctions with spatial and semantic properties, while at the same time being simple enough.

\paragraph{Challenges \& Methodology.}

With input constraints such as boundaries and room requirements, our goal is to generate high-quality vector floorplans. 
%
Floorplans have a complex structure containing elements ranging from the low-level to the high-level such as wall junctions, wall segments, and room polygons, which poses two challenges. 
%
On the one hand, high-level elements may share low-level elements, leading to complex geometric and topological dependencies between elements. It is challenging to design a model that can handle these complex dependencies. 
%
On the other hand, the structural and semantic attributes of vector floorplans are not independent, which poses another challenge in designing a model for learning structural-semantic dependencies.

In this paper, we propose the following methodology to solve these challenges. To address the complexity of floorplan structure, we transform the vector floorplan generation problem into a graph generation task, by representing the vector floorplan as a structural graph \(G = (V, E)\). This task requires estimating the data distribution of structural graphs for sampling, but the distribution is pretty complex. 
%
As mentioned above, vector floorplans have multi-level structures and generating all 0D wall junctions basically determines the whole floorplan structures. To tackle the challenge of structural and semantic dependency, we co-learning them by considering them both as node attributes. To this end, we propose a novel generative model,~\textit{StructDiffusion}, to decouple the structure graph generation into two stages: node generation and edge prediction. The overview of our framework is illustrated in Figure~\ref{fig:teaser}. 
%
Node generation involves estimating and sampling the joint probability density \(P(V)\) of the node set, while edge prediction involves predicting \(P(E|V)\) based on the generated node set to obtain \(E\), resulting in the complete structural graph \(G = (V, E)\). Finally, all minimal polygonal loop of the structural graph are extracted as rooms to obtain the final vector floorplan.
